Blockchain-Enhanced Framework for Secure Third-Party Vendor Risk Management and Vigilant Security Controls

In an era of heightened digital interconnectedness, businesses increasingly rely on third-party vendors to enhance their operational capabilities. However, this growing dependency introduces significant security risks, making it crucial to develop a robust framework to mitigate potential vulnerabilities. This paper proposes a comprehensive secure framework for managing third-party vendor risk, integrating blockchain technology to ensure transparency, traceability, and immutability in vendor assessments and interactions. By leveraging blockchain, the framework enhances the integrity of vendor security audits, ensuring that vendor assessments remain up-to-date and tamperproof. This proposed framework leverages smart contracts to reduce human error while ensuring real-time monitoring of compliance and security controls. By evaluating critical security controls-such as data encryption, access control mechanisms, multi-factor authentication, and zero-trust architecture-this approach strengthens an organization's defense against emerging cyber threats. Additionally, continuous monitoring enabled by blockchain ensures the immutability and transparency of vendor compliance processes. In this paper, a case study on iHealth's transition to AWS Cloud demonstrates the practical implementation of the framework, showing a significant reduction in vulnerabilities and marked improvement in incident response times. Through the adoption of this blockchain-enabled approach, organizations can mitigate vendor risks, streamline compliance, and enhance their overall security posture.

==> Implementation.tex <==
\section{Implementation}

\label{implementation}


A zero-day attack vulnerability is a type of threat that takes advantage of a previously undiscovered weakness in a computer application. This exploit is initiated instantly, with no time gap between discovering the weakness and mounting a defense against the attack~\cite{bu2014zero}. Therefore, it is challenging to identify the potential issues that can lead to zero-day attacks. Presenting a zero-day attack security threat assessment for a third-party vendor involves a structured and comprehensive approach to ensure clarity and actionable insights. The process begins with an introduction that outlines the objective of evaluating the vendor's preparedness and resilience against zero-day attacks, followed by defining the scope of the assessment. A detailed overview of the zero-day attack landscape is provided, including definitions, current trends, statistics, and notable incidents relevant to the vendor's industry. The assessment methodology is then explained, detailing the specific tools and techniques used, such as penetration testing, vulnerability scanning, and threat modeling. The evaluation of existing security controls includes a review of preventive measures like firewalls and intrusion prevention systems, detection mechanisms such as intrusion detection systems and behavioral analytics, and response strategies including incident response plans and patch management. The findings section summarizes the vulnerabilities identified and assesses their potential impact on the vendor’s operations and data security. Based on these findings, immediate actionable recommendations are provided, focusing on enhancing patch management, integrating threat intelligence, and conducting regular security awareness training. Long-term strategies, such as implementing a zero trust security model, scheduling regular audits, and investing in advanced threat detection technologies, are also suggested to bolster the overall security posture. An implementation plan is outlined, including a timeline for executing the recommended measures, the resources required, and the monitoring metrics to assess their effectiveness. This proposed framework provide possible security controls that can mitigate the risk of Zero-day attacks are listed as follows:\\

 \begin{itemize}
 \item
 
Maintaining a list of authorized and unauthorized devices and softwares: Maintain an inventory of both the authorized devices and software in the system. In addition to that, blacklist the unauthorized devices and software to mitigate the probable risk associated with them. In this way, only executing solely approved and trusted applications on systems is allowed, thereby limiting the running of unauthorized or potentially malicious software.\\
\item Maintenance and analysis of audit logs:  System call auditing is carried out on every active process running on each individual host in the entire system. This comprehensive approach is necessary because predicting the specific process involved in attacks is challenging. It is possible to ignore or miss system calls associated with vulnerabilities if one only concentrates on auditing limited process system calls. System calls related to socket communications, OS operations, and timestamps for each system call are potential source of information for determining if a system call and its associated objects are involved in malicious spread. \\
\item Limit and control network configuration:  
 Secure configuration of network devices such as routers and switches and utilizing firewalls to filter and manage both incoming and outgoing network traffic creates a boundary defense. Regular review and update of the firewall rules are also necessary to enhance security. Furthermore, building Access Control Lists facilitates controlling and restricting access to specific IP addresses, ports, and services on the vendor's network. Additionally, employ network segmentation to isolate components specific to the vendor, restricting their access to critical resources. Finally, conducting penetration tests and managing incident responses through continuous vulnerability assessments helps mitigate the risk of zero-day attacks.
 \\
\begin{figure}
\centering
 \includegraphics[width=8cm, height=3cm\columnwidth]{Bayes.jpg}
\centering
\caption{Bayesian Network with  Conditional Probability Table}
\label{Bayed}
\end{figure}
 

\item Building a Bayesian model to capture the attack path: Graphical models known as Bayesian Networks use probability to depict cause-and-effect interactions. They are described as directed acyclic graphs (DAG) where each node represents a variable, and the causal relationship between two variables is indicated by an edge~\cite{ sun2018using}. A simple Bayesian Network with a Conditional Probability Table is depicted in Fig~\ref{Bayed}. It states that the probability of Burglary being true is .9 when the house alarm is activated, and it is true. In this way, a conditional probability relationship between any two events can be inferred based on the information in the Bayesian Network and the associated Conditional Probability Table.\\


Build a Bayesian network where each node represents the entities and components, for example, system calls, application programs, network connections, servers, and users in the system, and each edge indicates the conditional probabilities between two nodes. For instance, the conditional probabilities between two nodes can be expressed as the compromise of a particular node, which may depend on another node's condition or specific security measures. Next, assign a probability of being compromised or a security measure being breached for each node in the network. After that, compute the probabilities associated with various nodes or paths based on the evidence that has been observed leveraging the Bayesian inference rule~\cite{dempster1968generalization}. Log entries, alerts, or other indicators of being infected or compromised can be evidenced in the model. Analyze the probabilistic outcome of the Bayesian network to identify the most probable paths of attack or crucial nodes in the system. This information aids in prioritizing security measures and responding effectively. Establishing connections between high-probability instances through dependency relations forms a path representing the zero-day attack path. For efficient performance, the Bayesian network must be updated with new evidence or observations.



 \end{itemize}


==> Privacy.tex <==
\section{Privacy Considerations for Third-Party Assessment}
\label{privacy}

As artificial intelligence (AI) continues to advance, there are growing concerns about ethical issues. AI technology is rapidly evolving and expanding its presence, from virtual assistants like Alexa and Google to smart vehicles and facial recognition systems. However, the use of AI technology raises privacy concerns, particularly regarding personal data. The collection and processing of this data can raise worries about how it is being used and who has access to it. The primary privacy issues in AI include the potential for unauthorized data access and breaches of confidential personal information. With vast amounts of data being collected and analyzed, there is a risk of it falling into the wrong hands through security breaches or hacking. As AI advances, it also raises concerns about the misuse of personal information, leading to an increase in data breach incidents. Generative AI can be misused to create fake profiles or manipulate images. Like all other AI technologies, generative AI relies on data. Cybercrimes impact the security of corporations worldwide, and the mishandling of personal data can have serious consequences. It is crucial to implement robust data protection measures to mitigate the potential risks of AI, including enforcing access controls, implementing data protection laws, encrypting sensitive data, and monitoring systems for unauthorized access. Additionally, AI systems should be designed with privacy in mind, and data should only be managed and used for legitimate purposes. Ultimately, it is essential to promote the responsible development and deployment of AI to harness its potential benefits while minimizing threats to individual privacy.



==> Threat.tex <==
\begin{table*}[btp]
\caption{Vendor Assessment Questions}
\label{table2}
\begin{center}
\begin{tabular}{ |p{15cm}| } 
 \hline
What compliance certifications does AWS hold relevant to healthcare, such as HIPAA, HITRUST, or GDPR?\\
Can AWS provide documentation or reports on their compliance with these standards?\\
How does AWS ensure the privacy and protection of healthcare data?\\
What measures are in place to maintain data confidentiality, integrity, and availability?\\
Where will our healthcare data be stored geographically?\\
Are there options to choose specific data residency to comply with local healthcare data regulations?\\
How does AWS manage access control for both internal and external users?\\
What authentication and authorization methods are supported, such as multi-factor authentication (MFA) and role-based access control (RBAC)?\\
What identity and access management (IAM) solutions does AWS offer?\\
How are user credentials and permissions managed to prevent unauthorized access?\\
How does AWS handle data encryption at rest and in transit?\\
Are there options for customer-managed encryption keys or hardware security modules (HSMs)?\\
What data backup and disaster recovery options are available?\\
How frequently are backups performed, and what is the recovery time objective (RTO) in case of a failure?\\
What network security measures does AWS implement, such as firewalls and intrusion detection/prevention systems (IDS/IPS)?\\
How is network traffic monitored and controlled within the AWS infrastructure?\\
How does AWS ensure the isolation of our data and workloads from other customers?\\
What measures are in place to prevent cross-tenant access in a multi-tenant environment?\\
What is AWS’s incident response policy and process?\\
How are customers notified and supported in the event of a security breach?\\
What security monitoring and logging services does AWS provide?\\
How can we access and analyze logs for compliance and auditing purposes?\\
Does AWS undergo regular third-party security audits?\\
Can AWS provide recent audit reports or summaries relevant to healthcare?\\
What are the specific security responsibilities of AWS versus those of the customer under the shared responsibility model?\\
How does AWS support healthcare organizations in meeting their security obligations?\\
What physical security measures are in place at AWS data centers?\\
Can AWS provide details on data center access controls, surveillance, and environmental safeguards?\\
How does AWS handle vulnerability management and patching for their infrastructure and services?\\
What is the process for reporting and addressing vulnerabilities in AWS services?\\
Does AWS conduct regular penetration testing of their infrastructure?\\
Are customers allowed to perform their own penetration tests on their AWS environments?\\
What legal protections and liability clauses are included in the contract with AWS?\\
How does AWS handle data requests from law enforcement or government agencies, particularly for sensitive healthcare data?\\
How does AWS handle the security of IoT devices connected to their cloud services?\\
What measures are in place to ensure secure communication between IoT devices and the cloud?\\
How does AWS secure edge computing solutions that may be used in conjunction with IoT devices?\\
What safeguards are in place to protect data processed at the edge before it reaches the cloud?\\
What specific measures does AWS take to protect patient data in compliance with healthcare regulations?\\
How does AWS ensure the integrity and confidentiality of electronic health records (EHRs) and other sensitive patient information?\\

 \hline
\end{tabular}
\end{center}
\end{table*}


